Attention-based Dual-stream Vision Transformer for Radar Gait Recognition

Radar gait recognition is robust to light variations and less infringement on privacy. Previous studies often utilize either spectrograms or cadence velocity diagrams. While the former shows the time-frequency patterns, the latter encodes the repetitive frequency patterns. In this work, a dual-stream neural network with attention-based fusion is proposed to fully aggregate the discriminant information from these two representations. The both streams are designed based on the Vision Transformer, which well captures the gait characteristics embedded in these representations. The proposed method is validated on a large benchmark dataset for radar gait recognition, which shows that it significantly outperforms state-of-the-art solutions.

==> aintroduction.tex <==
% background introduction & importance of this work.
Human gait recognition has become increasingly attractive in biometrics with many applications such as public safety monitoring, health screening and human-computer interaction \cite{zhang2018latern}. Traditional gait recognition methods~\cite{liao2020model,zhang2016siamese} often require videos captured in a side view and heavily depend on the lighting conditions. The photos of people may also raise privacy concerns. In contrast, continuous-wave (CW) radar can capture the micro-Doppler signatures (mDS) of front-view gait features from a moving target \cite{addabbo2021temporal}, reveal human dynamic features and detect human motions and gestures \cite{addabbo2021temporal,bai2019radar,le2018human}. More importantly, the radar signal is less invasive of privacy and can work in dim-light conditions, ensuring robustness in a variety of real-world situations. In this paper, we analyze the radar mDS for front-view human gait recognition.
% todo mDS signals

% analysis of spectrogram and cvd
Many energetic representations of mDS analysis have been developed, e.g. spectrograms~\cite{ren2017regularized,ren2021three}, cadence velocity diagrams (CVD)~\cite{} and cepstrograms~\cite{}. The spectrogram is a time-varying representation of mDS in the joint time-frequency domain \cite{addabbo2021temporal}, which has been applied to human activity recognition~\cite{le2018human,kim2015human}. The time-varying gait information such as the swinging speed of arms and legs can be well encoded in the spectrogram. However, the gait spectrograms of different people have very little difference, while the same person may have different gait characteristics, which makes the radar gait recognition particularly challenging. 

% The repetition information of those frequencies is scarcely considered but is also the invariant feature of gait cycles.
The CVD is another form of mDS representations by taking Fast Fourier Transform of the spectrogram along the time axis~\cite{bjorklund2012evaluation}. The CVD is less studied for gait recognition~\cite{seifert2017new}, but it provides a useful measurement of repetition pattern for different velocities of body parts, which provides complementary information to the spectrogram. 

% fusion
% Feature fusion is a common practice in deep learning models in order to improve the classification performance when more than one streams or channels are involved. It can be classified to score-level fusion and feature-level fusion. Score-level fusion only considers the probability vectors. Feature-level fusion, which aims to utilising all or part of features from different sources, can be achieved by concatenation, averaging, max pooling, min pooling, etc. Attention-based feature-level fusion is another approach which could memorising the relationship and decide the importance and confidence of both features and therefore provide more promising results \cite{yang2017neural}.

% classification learning methods
Traditional classifiers such as Na\"{i}ve Bayes~\cite{fioranelli2016centroid}, support vector machines~\cite{begg2005support} and $k$-nearest neighbours~\cite{van2017classification} have been used to classify mDS, while deep convolutional neural networks (DCNNs) often produce better performance. DCNNs have been used on spectrograms for radar-based gesture recognition and action classification \cite{addabbo2021temporal,le2018human,cao2018radar}. Other representations such as CVD could provide complementary information to spectrogram, and their use of DCNNs often ignore the unique physical nature of radar signal representations compared to optical images. 

% how to solve the problem
In this work, an Attention-based Dual-Stream Vision Transformer (ADS-ViT) is proposed to recognize people through gait mDS. As spectrograms often focus on the short-time-varying nature of mDS only, the CVD is introduced to capture the information on how often different frequencies repeat across a long duration. The proposed dual-stream network could extract features from these two representations simultaneously, where each stream is designed based on vision transformer (ViT) to utilize the patching function to deeply exploit the gait characteristics in spectrogram/CVD. Furthermore, an attention-based fusion is designed to combine features from two streams. The proposed framework is validated on a large dataset for radar gait recognition and significantly outperforms state-of-the-art models.

% summarise contributions
Our contributions are two-fold: 1) The proposed ADS-ViT could effectively extract and fuse features from spectrogram and CVD for radar gait recognition. 2) Each stream of ADS-ViT could utilize the patch-processing ability of ViT to effectively capture the gait characteristics embedded in patches corresponding to frequency bands of spectrogram/CVD.

% The remainder of the paper is structured as follows. Section II demonstrates the proposed method of the attention based dual-stream Vision Transformer in radar signal processing and classification. Section III shows the experimental results with analysis, illustrating the performance of our approach. Section IV presents the conclusion.


==> cexperiental.tex <==

% To illustrate the classification ability of our proposed method attention-based AT-DSViT, we evaluate several latest neural networks  MobileNet \cite{ sandler2018mobilenetv2}, Vision Tranformer (ViT) \cite{dosovitskiy2020image} and our model for ablation study. The results show promising performance of our model, achieving an accuracy of 91.02\% in our dataset. We also compare the proposed attention-based fusion with several state-of-the-art methods using VGG \cite{simonyan2014very}, AlexNet \cite{krizhevsky2012imagenet} and ResNet \cite{he2016deep}, and find our approach able to perform better in aggregating two radar signal representations.

\subsection{Dataset overview}
\label{sssec:dataset}
The evaluation is based on a gait dataset collected by authors, which consists of 1669 walking sequences from 98 volunteers. To enable the detection ability under different clothing conditions, we deliberately invite volunteers to come for the data collection twice on different days. However, the route and distance those volunteers undergo are carefully assured fixed. Volunteers walk naturally from one end to the other, towards the Doppler radar, then turn around and walk to the origin. The whole walking process mentioned above is a complete sequence which lasts about 30 seconds. Each member has walked 10 sequences for both data collection events, but some have only joined the first or the second. \textcolor{red}{\{Following describes segmentation, each person has 200 to 300 segments\}} Since the sequence could be long in the time axis, we crop each spectrogram into multiple frames (frame size is $115\times115$) with overlapping 0.2 seconds approximately representing a subject’s one complete gait cycle. For the consistency of all pieces of training, we deliberately generate a fixed training set randomly split from the whole dataset and let the remaining be the testing set. 
The ratio of data split is approximately 50\% to 50\%, containing 22,894 images for training and 22,874 for testing.

\subsection{Experimental settings}
\label{sssec:modelVariants}
We use the ViT with $16\times16$ input patch size as both the ViT model for direct training and the backbone of the proposed AT-DSViT. The parameter details of the applied ViT model is shown in Table \ref{vitbase}. We also choose the original AlexNet \cite{krizhevsky2012imagenet}, VGG16 \cite{simonyan2014very}, ResNet18 \cite{he2016deep},  MobileNetV2 \cite{ sandler2018mobilenetv2} and ViT-Base \cite{dosovitskiy2020image} models as the baseline CNNs for comparison. AlexNet has been used as backbone in \cite{cao2018radar} to identify humans and achieves leading performance. \cite{addabbo2021temporal} has considered VGG16 and ResNet18 as state-of-the-art methods in gait recognition tasks for comparison.

\begin{table}[htbp]
\centering
\caption{Variants details of Vision Transformer Base}
\label{vitbase}
\begin{tabular}{lllll}
\hline
Model    & Layers & Hidden size & MLP size & Heads \\ \hline
ViT-Base & 12     & 768         & 3072     & 12    \\ \hline
\end{tabular}
\end{table}

% \subsection{Training}
% \label{sssec:training}
% We train all three models using the aforementioned fixed training set and evaluate their performance with the testing set on an environment with two GeForce RTX 2080 Ti (12GB). All the signal and image processing, including the generation of CVD and concatenation of two representations, is conducted before feeding to the network. 
The input size is initially $115\times115$ and is resized to $224\times224$ to fit the adopted networks. SGD is the optimiser of all these models with a momentum of $0.9$ and weight decay of $5\times10^{-5}$. We take cross-entropy loss as the loss function. As for the learning parameters, a linear learning rate warmup and decay is used with a learning rate scheduler, and the initial learning rate is set to $0.01$ for ViT and ResNet, $0.001$ for AlexNet and $0.0001$ for VGG. The batch size is 128 for all training. The proposed AT-DSViT loads two pre-trained ViT weights for both spectrogram and CVD streams. All the models are trained for 500 epochs each.

\subsection{Performance comparison}
\label{sssec:comcnn}
\begin{table}[pt]
    \centering
    \caption{Accuracy comparison between of the state-of-the-art methods \cite{addabbo2021temporal,cao2018radar}. We also apply two benchmark object recognition models, MobileNet \cite{ sandler2018mobilenetv2} and ViT \cite{dosovitskiy2020image}, to the proposed radar gait recognition task. The experiments are run among single features (spectrogram or CVD) or feature fusion by the proposed AT-DSViT. }
    \resizebox{\hsize}{!}{
    \begin{tabular}{l|l}
        \hline\hline
        Method  &  Accuracy \\ 
   
        \hline
        DCNN-AlexNet on Spectrogram \cite{cao2018radar} & 71.56\% \\ 
        TCN-VGG16 on Spectrogram \cite{addabbo2021temporal}  & 69.24\%\\
        TCN-ResNet18 on Spectrogram \cite{addabbo2021temporal}   & 85.56\% \\
        \hline\hline
        DCNN-AlexNet on CVD &   72.44\% \\ 
        TCN-VGG16 on CVD &   79.83\%  \\ 
        TCN-ResNet18 on CVD &   80.73\% \\ 
        MobileNet on Spectrogram &   79.51\% \\ 
        MobileNet on CVD  & 76.84\%\\
        \hline\hline
        ViT-base 16x16 on Spectrogram  & 90.03\% \\
        ViT-base 16x16 on CVD &   80.14\% \\ 
        \textbf{Proposed AT-DSViT} & \textbf{91.02\%} \\ 
        \hline\hline
    \end{tabular}
    }
    \label{tab:results}
\end{table}

We conduct experiments to verify our approach with other state-of-the-art methods existing in the radar-signal-based recognition field. The comparison is demonstrated in Table \ref{tab:results}. AlexNet \cite{krizhevsky2012imagenet} has been used in earlier mDS human identification \cite{cao2018radar}, while VGG \cite{simonyan2014very} and ResNet \cite{he2016deep} are also commonly utilized in mDS human identification tasks more recently.  \cite{addabbo2021temporal} has used VGG and ResNet as state-of-the-art methods for comparison. In the experiments, AlexNet classifies around 72\% of targets successfully on spectrogram representations, while VGG16 perform worse on spectrograms with accuracy of 69.24\%. ResNet18, however, obtains the state-of-the-art with 85.56\% on spectrograms. Additionally, experiments are conducted on CVDs using three aforementioned SOTA methods, where the ResNet18 reaches the highest with classification accuracy of 80.73\%. 

We also conduct experiments on two commonly used object detection models, MobileNet \cite{ sandler2018mobilenetv2} and Vision Transformer (ViT) \cite{dosovitskiy2020image}. MobileNet \cite{ sandler2018mobilenetv2} is a light-weighted convolutional neural network that performs well on natural image tasks, and ViT \cite{dosovitskiy2020image} uses patching and transformer encoder to enable a suitable network for radar signal representations. 
% Due to the two-dimension nature of both the spectrogram and CVD, these representations have their own physical meaning according to the two axes.
Due to the spectrogram and CVD have different physical meaning along two axes, i.e. time-frequency and frequency-frequency, extracting features simply by convoluting on the entire figure in a monolithic CNNs would be insufficient and ignore portions of the physical information. In contrast, ViT could have promising potentials to perform better on such radar signal diagrams by patching and utilising the self-attention mechanism. It is clear to see that ViT achieves 90.03\% and outperforms the MobileNet in the spectrogram set by about 10\%, proving that ViT could extract more useful physical information than CNNs which use convolutional kernels to extract features. As for the CVDs, performances of the two networks do not vary considerably, with ViT achieving a slightly better performance (80.14\%) than the MobileNet (79.51\%). Compared to the methods above, the proposed AT-DSViT with attention-based fusion mechanism performs significantly better with an accuracy of 91.02\%. It can be concluded from the experimental results that the proposed AT-DSViT achieves a promising performance compared to the three state-of-the-art methods and thus is a suitable approach in human gait recognition tasks using mDS. 

% \begin{table}[htbp]
% \centering
% \caption{Classification results of backbone model comparison with two baseline CNNs. ViT outperforms MobileNet in both CVD and spectrogram set. }
% \label{table:ablation}
% \begin{tabular}{lll}
% \hline
% \textbf{Feature}             & \textbf{Model} & \textbf{Accuracy} \\ \hline
% \multirow{2}{*}{CVD}         & MobileNetV2 \cite{ sandler2018mobilenetv2}    & 79.51\%           \\ \cline{2-3} 
%                              & ViT-Base 16x16 \cite{dosovitskiy2020image} & 80.14\%           \\ \hline
% \multirow{2}{*}{Spectrogram} & MobileNetV2    & 76.84\%           \\ \cline{2-3} 
%                              & ViT-Base 16x16 & 90.03\%           \\ \hline
% Feature Fusion               & \textbf{AT-DSViT} & \textbf{91.02\%}  \\ \hline
% \end{tabular}
% \end{table}

% \subsubsection{Comparison to State-of-the-art Methods}
% \label{sssec:comcon}


% \begin{table}[htbp]
% \centering
% \caption{Comparison with three state-of-the-art methods, AlexNet, VGG and ResNet. }
% \label{table:sota}
% \begin{tabular}{lll}
% \hline
% \textbf{Feature}             & \textbf{Model} & \textbf{Accuracy} \\ \hline
% \multirow{3}{*}{CVD}         & AlexNet \cite{cao2018radar}       & 72.44\%           \\ \cline{2-3} 
%                              & VGG16 \cite{addabbo2021temporal}         & 79.83\%           \\ \cline{2-3} 
%                              & ResNet18 \cite{addabbo2021temporal}      &  80.73\%           \\ \hline
% \multirow{3}{*}{Spectrogram} & AlexNet        & 71.65\%           \\ \cline{2-3} 
%                              & VGG16          & 69.24\%           \\ \cline{2-3} 
%                              & ResNet18       & 85.56\%           \\ \hline
% Feature Fusion               & \textbf{AT-DSViT} & \textbf{91.02\%}  \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[htbp]
% \centering
% \caption{Comparison between the performance of five models using single feature in spectrogram or CVD dataset, and our attention-based dual-stream ViT. The fist three models, AlexNet, VGG and ResNet, are state-of-the-art methods, and the  experiments on MobileNet and ViT are conducted for ablation study. }
% \label{table:sota}
% \label{table:ablation}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{}               & \multirow{2}{*}{\textbf{Model}}                             & \multicolumn{2}{l|}{\textbf{Classification Accuracy}} \\ \cline{3-4} 
%                                 &                                                             & \textbf{Spectrogram}          & \textbf{CVD}          \\ \hline
% \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Single\\ Feature\end{tabular}} & AlexNet \cite{cao2018radar}                & 71.56\%                       & 72.44\%               \\ \cline{2-4} 
%                                 & VGG16 \cite{addabbo2021temporal}           & 69.24\%                       & 79.83\%               \\ \cline{2-4} 
%                                 & ResNet18 \cite{addabbo2021temporal}        & 85.56\%                       & 80.73\%               \\ \cline{2-4} 
%                                 & MobileNetV2 \cite{ sandler2018mobilenetv2}    & 76.84\%                       & 79.51\%               \\ \cline{2-4} 
%                                 & ViT-Base 16x16 \cite{dosovitskiy2020image} & 90.03\%                       & 80.14\%               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Feature\\ Fusion\end{tabular}                  & \textbf{AT-DSViT}                                              & \multicolumn{2}{c|}{\textbf{91.02\%}}                 \\ \hline
% \end{tabular}
% \end{table}


==> econclusion.tex <==
In this paper, we propose a novel approach to address the gait recognition problem. Gait feature can be captured by Doppler radars, and the signal can be represented as a time-frequency spectrogram as well as a cadence velocity diagram. The complementary nature of these two representations inspired us to develop a dual-stream Vision Transformer to take both features for better classification performance. Moreover, we utilise the attention based fusion to deeply extract and fuse useful features from the two representations. The use of Vision Transformer also enable the model to exploit the deep physical knowledge of radar signal, and the whole model is validated in our dataset. We conduct experiments to compare with baseline CNNs, and the result confirms that our model is suitable for the classification tasks of gait and the proposed attention based fusion works well in radar feature aggregation.

==> pic/bmethodology.tex <==
 \begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.98\textwidth]{pic/block diagram.png}
    \caption{(A) shows the overview of the whole architecture; (B) details the pipeline of ViT by illustrating its position and patch embedding and transformer encoder.}
    \label{fig:block}
\end{figure*}

% Due to the different representations of time-frequency spectrogram and CVD, they could have complementary identification features about a walking person. In the area of gait recognition, researchers often use only one feature representation in the classification task, while there exist various fusion methods such as simple concatenation, score-level fusion, etc. to integrate features from different representations \cite{chen2019attention}. Attention mechanism has been suggested to be powerful in focusing on the important part which provides abundance information in specific feature maps. In our work, we are inspired by \cite{chen2019attention} to propose an attention-based fusion method for fusing deep features of time-frequency spectrogram and CVD in order to make the best use of them. Moreover, we propose to use Vision Transformer based dual-stream neural network in extracting features from the two representations.

% The block diagram of this proposed method is shown in Figure 1, which consists of four main steps. Time-frequency spectrograms are fist generated from raw radar signal and CVDs are then converted from the generated time-frequency spectrograms. After the whole dataset is generated completely, spectrograms and CVDs would be fed into two separate ViT stream for extracting their own features. Attention-based fusion mechanism is then applied to find the most useful features from two and fuse them into one feature map. Finally, a fully-connected layer would transfer the feature map into the classification message.


\subsection{Time-frequency representations}
\label{sssec:complementary}
\emph{Spectrogram:} Tahmoush and Silvious \cite{ seifert2017new} have modelled Doppler of each body part of a walking human as sinusoidal modulation in the spectrogram. The model reveals the velocities of each body part which is instrumental in determining the necessary human gait characteristics. The fundamental characteristics are the mean Doppler velocity and the size of the torso variation in the micro-Doppler. It has been found that the mDS of a person is relatively consistent and different walking people lead to clearly discriminative mDS \cite{seifert2017new}. Time-frequency spectrogram can well manifest such time-varying human gait characteristics. A sample spectrogram is shown in Fig.~\ref{fig:block}.

% To obtain the time-frequency spectrogram, our approach is to split the signal $s$ into narrow segments with overlap using a window function $w$ and apply Fourier transform to each of the segments \cite{yang2017time}. In this case, the spectral information of each time segment is obtained. Then, those corresponding segments are concatenated to derive the final spectrogram. The above process is also known as the short-time Fourier transform (STFT). The STFT procedure on signal $s(t)$ can be fomulated as 
% \begin{equation}
%     S(t,\omega) = \int_{-\infty}^{+\infty}s(t+\tau)w(t)e^{-j\omega\tau}dt
% \end{equation}
% The spectrogram is obtained as follow. The signal $s(t)$ is segmented into $M$ overlapping frames $\{\boldsymbol{x}_0, \boldsymbol{x}_1, . . . , \boldsymbol{x}_{M-1}\}$, where each frame $\boldsymbol{x}_i = \{x_i[n], n = 0, 1, . . . , N - 1\}$ is a column vector of length $N$. These $M$ frames form a synthetic image $\boldsymbol{X} = [\boldsymbol{x}_{1}, ... , \boldsymbol{x}_{M-1}]$ of size $M \times N$. Then, the discrete Fourier transform $\boldsymbol{f}_i = [f_{i,0}, f_{i,1},..., f_{i,N-1}]$ of $\boldsymbol{x}_i$, $\boldsymbol{f}_i=\mathcal{F}\{\boldsymbol{x}_i\}$ is computed as:

% \begin{equation}
% f_{i, k}=\sum_{n=0}^{N-1} x_{i}[n] \exp \left\{-j 2 \pi \frac{k n}{N}\right\},
% \end{equation}
% where $\mathcal{F}\{\cdot\}$ denotes the Fourier transform. The magnitude $\boldsymbol{S}=\{|\boldsymbol{f}_{i,k}|^2,i=0,\dots,M-1,k=0,\dots,N-1\}$ forms the spectrogram of size $M\times N$. 

\noindent \emph{Cadence velocity diagram (CVD):} The cadence velocity diagram has been proposed by \cite{bjorklund2012evaluation} to analyse micro-Doppler signatures. After deriving the spectrogram, the CVD is obtained by taking the Fourier transform on the spectrogram along the time dimension for each Doppler frequency bin. The derived CVD, as shown in Fig.~\ref{fig:block}, is a matrix with rows containing Doppler frequency (i.e. target velocity) and columns containing cadence frequency, which measures how frequently different frequencies appear in the signal over time. In other words, it illustrates the useful information of the repetition of velocities, which would be another key identification feature of a walking person. 
%As a result, the CVD provides data on the shape, size, and frequency of the curves in the original spectrogram. 



\subsection{Attention-based Dual-stream Vision Transformer}
\label{sssec:AT-DSViT}
Since two representations are used to provide different features, it is common to train two feature extraction networks for both of them. We therefore propose an attention-based dual-stream Vision Transformer (AT-DSViT). An overview of this model is depicted in Fig.~\ref{fig:block}. The model consists of two separate but identical networks which are both ViTs. Two sub-networks are fed with time-frequency spectrograms and CVDs respectively and output their own feature maps for fusion afterwards. Both spectrogram and CVD are obtained before training. We choose Vision Transformer (ViT) \cite{dosovitskiy2020image} as the backbone of our network. 

The AT-DSViT network can be formulated into a quadruplet $Q = (I_{TFS}, I_{CVD}, F, C)$, where $I_{TFS}$ and $I_{CVD}$ are two input radar representations fed into the two ViT streams, $F$ is an attention-based fusion layer and $C$ is a classifier. Through the two ViT streams, features of two input representations would be extracted as output. Note that both input representations are resized in the same size of $224 \times 224$ with 3 channels which could be accepted by the ViTs, and since the two ViT streams are identical the resulting output would be in the same size as well. The process could be formulated as follow:
\begin{equation}
    f_{TFS} = ViT_{1}(I_{TFS}),
\end{equation}
\begin{equation}
    f_{CVD} = ViT_{2}(I_{CVD}).
\end{equation}
where $f_{TFS}$ and $f_{CVD}$ are feature maps of TFS and CVD in the size of $1 \times 192$.
Here we have made modification to the original ViT Base $16 \times 16$ model, changing the last fully-connected layer to a $768 \times 192$ matrix for extracting middle-level features.
The attention-based fusion layer would then take the two output feature maps and generate a fused feature $f_f$: 
\begin{equation}
    f_f = F(f_{TFS}, f_{CVD}).
\end{equation}
Classifier $C$ finally takes the fused feature $f_f$ and generate the classification message.



% \subsection{Backbone Vision Transformer}
% \label{sssec:ViT}
Compared to commonly used convolutional neural networks such as VGG \cite{simonyan2014very}, AlexNet \cite{krizhevsky2012imagenet}, MobileNet \cite{sandler2018mobilenetv2} and ResNet \cite{he2016deep}, Vision Transformer (ViT) \cite{dosovitskiy2020image} can reshape the spectrogram into several local patches and use attention mechanism to obtain global knowledge of patches. Unlike scenarios of real-world images where an object could be positioned anywhere in an image but mean the same, patches of spectrogram and CVD converted from radar signal have their unique physical meaning when positioned in different locations in a diagram. This is because each patch contains knowledge about its specific area according to its time and frequency dimension for spectrogram or frequency dimensions for CVD. Even patches similar in representation could be physically different based on their frequency levels and temporal position. Instead of convolutional kernels in CNN, patches are therefore ideally used to reserve the positional information of signal representations as well as the relationship between them. In our method, ViT is responsible for splitting diagrams in patches and embed their positions, and a multi-head attention mechanism in transformer encoder could further extract the reserved physical information, processing physical meanings in the same way as natural language.

The architecture of ViT is depicted in Fig. 1. The input picture is first split into 196 separating patches with a size of $16 \times 16$, and each patch is then flattened to a 768-length vector. Then classification tokens are concatenated and position embedding is conducted by adding a position matrix, resulting in an overall $197 \times 768$ matrix. The sequence of vectors are then fed to a standard transformer encoder, and this would be executed 12 times for the ViT base model. The transformer encoder module contains a multi-head self-attention layer, which is global and can process the relationship between patches. The output feature vector of transformer encoder after classification token extraction is in the size of $1 \times 768$. An MLP head is responsible for taking the above feature vector and classification.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{vit.png}
%     \caption{Architecture of Vision Transformer}
%     \label{fig:my_label}
% \end{figure}



\subsection{Attention-based fusion}
\label{sssec:attention}
Various fusion methods exist, such as score-level fusion, feature concatenation and feature averaging. We found none of these could extract core features from two representations deeply. Inspired by Chen \emph{et al.} \cite{chen2019attention}, we utilize an attention-based fusion architecture illustrated in Fig.~\ref{fig:block}(A) to perform the fusion task for two representations spectrogram and CVD. 

Since the attention-based fusion is feature-level, the ultimate job is to find a set of weights $w$ for the features we have $f$ to obtain an aggregated feature $f_a$:
\begin{equation}
    f_a=\sum_{i=1}^{n}w_if_i,
    \label{eq:aggregated}
\end{equation}
where $n$ is the number of features.

In the attention-based fusion model, only one parameter kernel $q$ is required to be trained. The process begins with a Hadamard product (element-wise multiplication) between the output feature vector and kernel $q$:
\begin{equation}
    p_i = q f_i,
\end{equation}
where $p$ is the pre-weight which represents the confidence scores, and $q$ has the same size as feature vector $f_i$.

A softmax function is then applied to convert the pre-weights $p$ to a normalized probability distribution:
\begin{equation}
    w_i=\frac{e^{p_i}}{\sum_{n}e^{p_n}},
\end{equation}
where $w_i$ is the final weight of feature $f_i$ and $n$ denotes the number of features.

The fused feature vector is finally generated by adding weighted features together using Eq.~\ref{eq:aggregated}. This attention-based fusion could well highlight the most useful features by training only one parameter.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{attention.png}
%     \caption{Attention based fusion}
%     \label{fig:my_label}
% \end{figure}

% \subsection{Segment based fusion after prediction}
% \label{ssec:fusion}


% \begin{figure}[htb]
% \begin{minipage}[b]{.4\linewidth}
%   \centering
%   \centerline{\includegraphics[width=3.0cm]{pic/8.PNG}}
% %  \vspace{1.5cm}
%   \centerline{(a) Sample Spectrogram}\medskip
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.4\linewidth}
%   \centering
%   \centerline{\includegraphics[width=3.0cm]{pic/5.PNG}}
% %  \vspace{1.5cm}
%   \centerline{(b) Sample CVD}\medskip
% \end{minipage}
% %
% \caption{Examples of spectrogram and CVD.}
% \label{fig:sample}
% %
% \end{figure}
